Poincar\'e Duality for Generalized Persistence Diagrams of (co)Filtrations

We dualize previous work on generalized persistence diagrams for filtrations to cofiltrations. When the underlying space is a manifold, we express this duality as a Poincar\'e duality between their generalized persistence diagrams. A heavy emphasis is placed on the recent discovery of functoriality of the generalized persistence diagram and its connection to Rota's Galois Connection Theorem.

==> reviewer_comments.tex <==
1. Page 2, Line10.  "..They define the persistence diagram as the
M¨obius inversion of the generalized rank invariant.  Unlike classical
persistence, these persistence diagrams have negative multiplicities.
This makes the question of stability very difficult as we can not use
existing methods for constructing a matching".  I don't see the point
here.  The persistence diagram obtained by the Birth-Death function
also has negative multiplicities.  Maybe emphasize the point about
stability.

****
We agree it's not clear what the point of that paragraph is as written. We modified a couple sentences. We added a line saying that the birth-death approach also produces negative multiplicities. 
****

2. Page 10, Line 29.  Calling a Galois connection of module morphisms
as module morphisms can be a bit confusing.  It is not clear to me
what is the relationship between the standard notion of morphisms of
modules f:M -> N and module morphisms (f,g) defined by the authors.  I
think morphisms defined by authors are not clear if they are a special
case of morphisms in the standard sense or vice versa.  If the two
notions are irrelevant to each other (the authors definition and the
standard one) then they should just call them Galois morphisms- or
Galois connection morphisms of modules (or something along those
lines).

***
We renamed the morphism between two persistence modules to module-preserving morphisms so that it is now consistent with "filtration-preserving morphisms" and "cofiltration-preserving morphisms" earlier in the paper. All three use Galois connections. We hope this clears up the confusion.
***

3. Proposition 5.3 is not clear to me why it implies that Mobius
inversions of the birth-death function of a module with respect to two
different presentations should be the same except in the diagonal.
This should be made more clear.  One can remedy this by showing a
separate result that (Int f)#δZBψ~δΖΒψ or have an additional
explanation.  An alternative way to show it can be, to show that
δKer_Μ is invariant (up to ~) of Galois connection morphisms of
modules and utilize that δKer_Μ~δΖΒφ (an argument along these lines).


***
We rewrote the statement of Proposition 5.3 so the claim is now explicit. In fact, we reordered the introduction of these concepts so that this subsection better matches Sections 3.3 and Sections 4.3.
***

4. "This makes G(a) a supcomplex.  Note that the open star of the
subdivision of F(a) in L is G(a).  This means that |F(a)| is a
deformation retract of |G(a)|." This property needs a proper citation.
Also would be nice if the authors define the notion of open star and
the notion of (barrycentric and more generally of) subdivision.  These
would make the proof more clear to the reader.

***
The notion of a barycentric subdivision is defined in the text. We added a citation to Munkres regarding the deformation retraction. We added a sentence describing the open star as well.

***

5. In the right hand-side of Figure 1 it would look nicer if the
connections in the lattice do not overlap.  This also happens in other
places in the paper (e.g Figure 5).  There should be a way to fix this
in Tikcd in LaTex (I am assuming the authors use Latex)\

***
We reworked all the figures to address the issue raised. We also
eliminated all information in figures that can easy be described in the caption. Our figures are more streamlined now.
***

6. Page 12, Line 11.  says -> implies

***
Done
***
